oo7: Low-overhead Defense against Spectre Attacks via Program Analysis

The Spectre vulnerability in modern processors has been widely reported. The key insight in this vulnerability is that speculative execution in processors can be misused to access the secrets. Subsequently, even though the speculatively executed instructions are squashed, the secret may linger in micro-architectural states such as cache, and can potentially be accessed by an attacker via side channels. In this paper, we propose oo7, a static analysis approach that can mitigate Spectre attacks by detecting potentially vulnerable code snippets in program binaries and protecting them against the attack by patching them. Our key contribution is to balance the concerns of effectiveness, analysis time and run-time overheads. We employ control flow extraction, taint analysis, and address analysis to detect tainted conditional branches and speculative memory accesses. oo7 can detect all fifteen purpose-built Spectre-vulnerable code patterns, whereas Microsoft compiler with Spectre mitigation option can only detect two of them. We also report the results of a large-scale study on applying oo7 to over 500 program binaries (average binary size 261 KB) from different real-world projects. We protect programs against Spectre attack by selectively inserting fences only at vulnerable conditional branches to prevent speculative execution. Our approach is experimentally observed to incur around 5.9% performance overheads on SPECint benchmarks.

==> 3.to3e.tex <==
%!TEX root =main.tex
\section{Meltdown-style Malware Detection}
\label{sec:to3e}

\begin{table*}[]
	\caption {The analysis time of Meltdown-style malware detection on SPECint} \label{tb:md}
	\resizebox{\linewidth}{!}{	
		\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
			\hline
			\textbf{Program}           & \textbf{perlbench} & \textbf{bzip2} & \textbf{gcc} & \textbf{mcf} & \textbf{gobmk} & \textbf{hmmer} & \textbf{sjeng} & \textbf{libquantum} & \textbf{h264ref} & \textbf{omnetpp} & \textbf{astar} & \textbf{xalancbmk} & \textbf{Avg.} \\ \hline
			\textbf{Analysis time (s)} & 3193            & 45          & 1672      & 12       & 628        & 212         & 205         & 49               & 448           & 17            & 30          & 424             & 578       \\ \hline
	\end{tabular}}
\end{table*}


Meltdown-like malware revolves around the idea of accessing
unauthorized memory via out-of-order or speculative execution. Subsequently,
the value from this memory read is leaked via a covert channel, such as cache.
Therefore, the crux of detecting such malware is to discover the existence
of an instruction sequence that may perform the aforementioned actions.
There exists a variety of covert channels via which a value can be leaked.
Cache is a low noise channel and a substantial number of cache side-channel
attacks are capable to leak sensitive data. For the sake of simplicity, our
following discussion is based on {\tt Prime+Probe}, one of the most effective and
practical cache timing attack. But it can easily be
modified to capture other type of cache side-channel attacks such as
{\tt Flush+Reload}~\cite{yarom2014flush+}.

\subsection{Detection Method}

\paragraph*{Detecting reads from unauthorized memory address or registers}

Let us assume $\mathit{X}_{sup}$ captures the set of memory locations or
registers that a user process is unauthorized to access. For Meltdown and
Foreshadow attacks (cf. Table~\ref{tb:list_all}), $\mathit{X}_{sup}$ spans
over the kernel memory and the enclave memory, respectively. For RSRR (Rogue System Register Read) and
LazyFP (cf. Table~\ref{tb:list_all}), $\mathit{X}_{sup}$ captures the set
of system registers and floating point registers, respectively.
To identify the reading of an unauthorized memory location (Meltdown and
Foreshadow attacks (cf. Table~\ref{tb:list_all})), we check for an unauthorized
memory access ($\mathit{UA}$) and an instruction to leak the secret
($\mathit{LS}$) accessed by $\mathit{UA}$ within the speculation window
$\mathit{SEW}$. The presence of such a pair of instructions
$\langle \mathit{UA}, \mathit{LS} \rangle$ can be formalized via the
following condition $\Phi_{secret}$:
%The following condition
%holds when an unauthorized value is loaded into memory:
{\small
\begin{equation}
\begin{split}
\label{eq:malware-secret-load}
\Phi_{secret} \left ( \mathit{UA}, \mathit{LS} \right )
\equiv \left ( \mathit{addr}(UA) \cup \mathit{reg}(UA) \right )
\cap \mathit{X}_{sup} \ne \phi
\\
\wedge \mathit{mem}(\mathit{LS})
\wedge \mathit{Dep}(\mathit{UA}, \mathit{addr(LS)})
\\
\wedge \Delta(\mathit{UA}, \mathit{LS}) \leq \mathit{SEW}
\end{split}
\end{equation}}
In Equation~\ref{eq:malware-secret-load}, statically computing
$\mathit{addr}(UA)$ involves value analysis~\cite{cc04}.
Finally, for Foreshadow-NG~\cite{weisse2018foreshadow} attack, the condition
$\mathit{addr}(UA) \cap \mathit{X}_{sup} \ne \phi$ always holds, as
$\mathit{X}_{sup}$ might point to any virtual address, yet trick the
virtual memory manager (VMM) to launch an unauthorized access to a
physical memory page. Thus, 
\SP does not attempt to identify malware containing potential Foreshadow-NG attack~\cite{weisse2018foreshadow}.

\paragraph*{Identifying {\tt Prime+Probe} cache attack}
The basic idea behind {\tt Prime+Probe} cache attack is to first load a set of
cache sets (prime phase) with attacker controlled data before launching
the unauthorized memory/register access, as discussed in the preceding paragraph. After
the unauthorized access, the attacker times the access to cache sets
loaded in the prime phase to determine the secret located in the
unauthorized memory/register location.


Let us assume that the set of cache sets primed and probed are $S_{prime}$
and $S_{probe}$, respectively. Clearly, for a successful {\tt Prime+Probe}
cache attack, $S_{prime} \cap S_{probe} \ne \phi$.
Consider one such cache set $s_i \in S_{prime} \cap S_{probe}$. We need to
check whether cache set $s_i$ is subjected to {\tt Prime+Probe}. An instruction
sequence $I_{pri}$ primes a full cache set $s_i$ if they fill up all the ways of
cache set $s_i$. This is formalized via the following condition:
%Thus, to detect the prime
%phase of cache set $s_i$, we check the presence of a sequence of instructions
%$I_{pri}$ with the following condition:
{\small
\begin{equation}
\label{eq:prime}
\begin{split}
& \Phi_{prime}^{s_i} \left (  I_{pri} \right ) \equiv
\mathit{iSeq}(I_{pri}) \wedge
\bigwedge_{inst \in I_{pri}} \mathit{mem}(inst)
\\
& \wedge
\bigwedge_{inst \in I_{pri}} \left ( \mathit{set}(\mathit{addr}(\mathit{inst})) = s_i \right )
\wedge
\left | \bigcup_{inst \in I_{pri}} \mathit{addr}(\mathit{inst}) \right | = \omega
\end{split}
\end{equation}}
where $\omega$ captures the size of a full cache set $s_i$ and the predicate
$\mathit{iSeq}$ is evaluated true if and only if the sequence of instructions,
as provided via its argument, appear along any valid control flow path.


%Priming a cache set $s_i$ can be captured
%via the following condition:
%{\scriptsize
%\begin{equation}
%\label{eq:prime}
%\Phi_{prime}^{s_i} \equiv
%\mathit{mem}(\mathit{inst}) \wedge \left ( \mathit{set}(\mathit{addr}(\mathit{inst})) = s_i \right )
%\end{equation}}
%where the memory instruction $inst$ accesses the cache set $s_i$.


Probing a cache set requires finding the time to access the cache set. Thus, each probe to cache
set $s_i$ can be captured via a sequence $\langle t_s, inst, t_e \rangle$ where
$t_s$ is an instruction to log the time before the probe, $inst$ is the access
to probed cache set $s_i$ and $t_e$ is an instruction to log the time after the
probe. An instruction sequence $I_{pro}$ probes a full cache set $s_i$ if
$I_{pro}$ involves a sequence of triplets of the form $\langle t_s, inst, t_e \rangle$
that also fill up all the ways of $s_i$. Thus, probing cache set $s_i$ is captured
via the following condition:
{\small
\begin{equation}
\label{eq:probe}
\begin{split}
& \Phi_{probe}^{s_i} \left (  I_{pro} \right ) \equiv
\mathit{iSeq}(I_{pro})
\\
& \wedge
\bigwedge_{\langle t_s, inst, t_e \rangle \in I_{pro}} \left (
\mathit{time}(t_s) \wedge \mathit{mem}(inst)  \wedge \mathit{time}(t_e) \right )
\\
& \wedge
\bigwedge_{\langle t_s, inst, t_e \rangle \in I_{pro}} \left ( \mathit{set}(\mathit{addr}(\mathit{inst})) = s_i \right )
\\
& \wedge
\left | \{ \mathit{addr}(\mathit{inst})\ |\ {\langle t_s, inst, t_e \rangle \in I_{pro}} \} \right | = \omega
\end{split}
\end{equation}}
To capture the timing of an access, an attacker can use either {\tt rdtsc} instruction or
OS-provided standard APIs.



%Similarly, for probing the cache, attacker times the access to cache set $s_i$. Specifically,
%if there exists a sequence of instructions $inst_{j-1}$, $inst_{j}$ and
%$inst_{j+1}$, then the following condition holds for probing the cache
%set $s_i$:
%{\scriptsize
%\begin{equation}
%\begin{split}
%\label{eq:probe}
%\Phi_{probe}^{s_i} \equiv
%& \mathit{time}(\mathit{inst}_{j-1}) \wedge \mathit{mem}(\mathit{inst}_j) \wedge
%\left ( \mathit{set}(\mathit{addr}(\mathit{inst}_j)) = s_i \right )
%\\
%& \wedge  \mathit{time}(\mathit{inst}_{j+1})
%\end{split}
%\end{equation}}


\paragraph*{Detecting the malware}
We detect malware containing potential Meltdown or Foreshadow attacks when our analysis identifies an instruction
sequence that involves priming a cache set $s_i$, launching an
unauthorized access and probing the cache set $s_i$. Consider such an
instruction sequence $I_{mal}$. Thus, $I_{mal}$ will contain a subsequence
$I_{pri}$ satisfying $\Phi_{prime}^{s_i}$, followed by a subsequence $I_{sec}$
satisfying $\Phi_{secret}(\mathit{UA}, \mathit{LS})$ and terminating in
a subsequence $I_{pro}$ satisfying $\Phi_{pro}^{s_i}$. This is formally
categorized as follows:
{\small
\begin{equation}
\boxed{
\begin{split}
\label{eq:malware}
& \Phi_{malware}^{s_i} \equiv \exists I_{mal}.\ \mathit{iSeq}(I_{mal})
\\
& \wedge \exists I_{pri}, I_{sec}, I_{pro}.\ \  \left (  I_{mal} = I_{pri} \odot I_{sec} \odot  I_{pro} \right )
\\
& \wedge \Phi_{prime}^{s_i}(I_{pri}) \wedge \left ( \exists\ \mathit{UA}, \mathit{LS}
\in I_{sec}.\ \Phi_{secret} \left ( \mathit{UA}, \mathit{LS} \right ) \right )
\\
& \wedge \Phi_{probe}^{s_i}(I_{pro})
\end{split}}
\end{equation}}
where $\odot$ is an ordered composition of instruction sequences. As $s_i$
is an arbitrary cache set in Equation~\ref{eq:malware}, it is a general solution to detect
the presence of {\tt Prime+Probe} via any (set of) cache sets.
%
%where $\mathit{Seq}$ is a predicate that holds if and only if there exists an instruction
%sequence that satisfies the input predicates of $\mathit{Seq}$. Therefore, the first line
%of $\Phi_{malware}$ captures the condition of priming a set of cache sets
%$\bigcup_{i=1}^{k} s_i$. Similarly, the third line of $\mathit{Seq}$ captures probing the
%same set of cache sets.
In general, checking $\Phi_{malware}^{s_i}$ involves value analysis, program dependency
analysis and reachability analysis using the program CFG. Finally, although
$\Phi_{malware}^{s_i}$ is demonstrated for {\tt Prime+Probe} attack here, it can easily be
modified to capture other type of cache side-channel attacks such as
{\tt Flush+Reload}~\cite{yarom2014flush+}.



%{\scriptsize
%\begin{equation}
%\boxed{
%\begin{split}
%\label{eq:malware}
%\Phi_{malware} \equiv
%\mathit{Seq} & \left (
%\mathit{Seq} \left (\Phi_{prime}^{s_1}, \Phi_{prime}^{s_2}, \ldots, \Phi_{prime}^{s_k} \right ), \right.
%\\
%&\ \Phi_{secret},
%\\
%&
%\left. \mathit{Seq} \left (\Phi_{probe}^{s_1}, \Phi_{probe}^{s_2}, \ldots, \Phi_{probe}^{s_k} \right ) \right )
%\end{split}}
%\end{equation}}



\subsection{Implementation}

We have designed the malware detection module on top of the 
Angr~\cite{shoshitaishvili2016state} tool.
%Angr is a python-based framework combining
%both static and dynamic symbolic analysis for the multi-architecture binary.
Specifically, we leverage the value set analysis capability of Angr to detect
malicious code fragments, as captured via the condition $\Phi_{malware}^{s_i}$
(cf. Equation~\ref{eq:malware}). A crucial step in the Meltdown-style malware is to leak sensitive data through a covert cache side-channel. Recent work, such as SCADET~\cite{sabbagh2018scadet} detects {\tt Prime+Probe} attack. 
Unlike SCADET, our detection does not only concern the {\em Prime} and {\em Probe} phase, but also the illegal memory or register accesses. 
% Moreover SCADET uses {\em intra-group} and {\em inter-group} thresholds to identify two groups of access for {\em Prime} and {\em probe}; this requires the tracking of a large number of addresses. As the {\em Prime} and {\em Probe} are tightly constructed in a short contiguous instruction sequence to improve attack accuracy, we only record and analyze the memory access inside a sliding window with size $W_s$. If a cluster of addresses in one sliding window occupies an entire cache set, then we treat the respective cluster as 
% {\em Prime} or {\em Probe} depending on whether an illegal access is
% identified (see Equations~\ref{eq:malware-secret-load}-\ref{eq:malware}).


% he {\tt Prime+Probe} attack in Spectre-style
% malware occurs in transient instruction sequences. Moreover, SCADET uses 


%Algorithm~\ref{alg:clustering} demonstrates our address clustering method
%with sliding window size $W_s$.
%%In this algorithm, a queue structure $Queue$ is used to to manage the
%%sliding windows which has the size $W_s$.
%$AddrMap[i]$ records a set of addresses that map to cache set $i$.
%%In this algorithm, only the memory
%%access instructions are analyzed (line 6).
%%When a memory access instruction
%%$inst$ was captured, its accessed memory address $addr(inst)$ is firstly put
%%in the $Queue$, and if the $addr(inst)$ is never put in the $AddrMap[i]$,
%%then put it in the $AddrMap[i]$ where $i$ is the cache set index calculated
%%by function $getCacheSet()$ indicates the cache set address $addr(inst)$ should
%%map.
%If $AddrMap[i]$ records $\omega$ different addresses (i.e. the size of
%a full cache set), then a cluster of addresses is identified within the
%record $C$.
%%
%Consider $c_1, c_2 \in C$ and both $c_1$ and $c_2$ hold addresses for
%the same cache set. If $c_1$ (respectively, $c_2$) resides before
%(respectively, after) loading the unauthorized value (cf.
%Equation~\ref{eq:malware-secret-load}), then we detect a Spectre-style
%malware via \SP.



%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
%{\small
%	\begin{algorithm}[t]
%		\sffamily\small
%		\sffamily\footnotesize
%		\sffamily\scriptsize
%		\begin{algorithmic}[1]
%			\Require $P$: {Program binary}
%			\Ensure $C$: {A set of clustered address}
%			\State $C \gets \emptyset$
%			\State $Queue \gets \emptyset$
%			\State $AddrMap[i] \gets \emptyset$ $;i \in [0, \#set-1]$
%			\State {Let $inst$ be the first instruction of $P$}
%			\While {$inst \neq exit$}
%			\If {$mem(inst)$}
%			\State $Queue.push\_back(addr(inst))$
%			\State $i \gets set(addr(inst))$
%			\If {$addr(inst) \notin AddrMap[i]$}
%			\State $AddrMap[i] \gets AddrMap[i] \cup \{addr(inst)\}$	
%			\EndIf
%			\If {$AddrMap[i].size = \omega$} /* $\omega$ is the size of a full cache set */
%			\State $C \gets C \cup AddrMap[i]$
%			\State $AddrMap[i].clear()$
%			\EndIf
%			\If {$Queue.size > W_s $}
%			\State $inst = Queue.pop\_front()$
%			\State $i \gets set(addr(inst))$
%			\State $AddrMap[i].remove(addr(inst))$
%			\EndIf
%			\EndIf
%			\EndWhile
%		\end{algorithmic}
%		\caption{Address clustering}
%		\label{alg:clustering}
%	\end{algorithm}
%}


\subsection{Meltdown Evaluation results}

Since there are no Meltdown-style malware has been found in the wild, we choose the Proof-of-Concept code of Meltdown to evaluate the effectiveness of our detection and use SPECint benchmark to evaluate the analysis time.

Our implementation can detect the Proof-of-Concept code of Meltdown~\cite{pocmeltdown} (using {\tt Flush+Reload} attack) and a {\tt Prime+Probe} version of Meltdown modified by us based on the  Proof-of-Concept code~\cite{pocmeltdown}. We use the same set of programs from the SPECint CPU benchmark suite~\cite{henning2006spec}
for evaluating the analysis time of Meltdown-like malware. The result is listed in Table~\ref{tb:md}. Our detection algorithm takes around 578 seconds on average for the SPEC benchmarks.

% The analysis time depends not only on the binary size, but also on the
% complexity of the program logic and the number of conditional jump
% instructions. %For the instance, even $444.namd$ has the largest binary size (326~KB),the analysis time is only 145.3s which is completely less than $433.milc$ (804.78) which has the binary size of 142~KB.









==> 4.meltdown.tex <==
\section{Combatting Meltdown}
\label{sec:meltdwon}

Meltdown is a recently discovered vulnerability which can exploit
the side effects of out-of-order-execution~\cite{Lipp2018meltdown}. Meltdown
does not rely on the software vulnerabilities and it can be launched directly
from the attacker code. We can easily adapt the machinery of \SP to detect meltdown
signatures in potentially attack code.

%This section is trying to identify malicious code for performing Meltdown in arbitrary binaries.

For launching Meltdown, the attacker aims to load value from a kernel
address $ka$. This, of course, would result in an exception. However,
exploiting the out-of-order paradigm of execution, the value from the
address $ka$ might already be brought into the cache before the
exception is raised. This cached value, then, can be ex-filtrated via
standard cache side-channel attacks (e.g. using a probe array {\tt array2}
in the Spectre code).

%and spreads the value of $ka$ to the cache side-channel, e.g using $ka$ as an index to access a probe array $pa$. Meanwhile, the classical cache side-channel attack is performed in parallel for reading the leaked data from the cache side-channel.
%So the malicious code should contain the following instruction sequence:
%$$ flush(a) \to b=load(ka) \to access(pa + b) \to RETSC$$
%where $flush(a)$ is a $flush$ instruction that flushes a cache line which contains address $a$. $b = load(ka)$ donates a load instruction that loads data from a kernel address $ka$ to a variable $b$. and $access(pa+b)$ can be a memory load or store instruction that works on address $pa + b$. The instruction $RETSC$ is used to read the CPU cycles for cache side-channel attack. For detecting the malicious code of Meltdown, the static analysis should capture the code pattern that satisfies the following  conditions:

Let us assume that $\mathit{KA}$ captures the set of sensitive addresses
that the attacker does not have permission to access. For example,
$\mathit{KA}$ might capture the set of kernel memory addresses. A
meltdown signature is detected if a load instruction $\mathit{L1}$
points to an address in $\mathit{KA}$ and a memory access
$\mathit{IM1}$ is data-dependent on $\mathit{L1}$. Specifically,
the detection of Meltdown is captured via the condition
$\Phi_{meltdown}$
{\small
\begin{equation}
\boxed{
	\label{eq:meltdown}
	\begin{split}
	\Phi_{meltdown} \equiv
	%flush() \wedge
	\\
	load(\mathit{L1}) \wedge mem(\mathit{IM1}) \wedge
	%\\
	%RETSC() \wedge
	\mathit{addr(L1)} \cap \mathit{KA} \ne \emptyset \wedge \mathit{Dep}(\mathit{L1}, \mathit{IM1})
	\end{split}}
\end{equation}}
%The first three line capture the malicious instruction sequence. The fourth line guarantees that the load operation is working an address from kernel. The last line ensures that the data from kernel is leaked to the cache side-channel.
where $\mathit{addr(L1)}$ captures the set of addresses accessed by load
instruction $\mathit{L1}$. We use value set analysis~\cite{shoshitaishvili2016state}
to detect the set of values/addresses accessed by an instruction. This computes
a sound over-approximation of $\mathit{addresss(L1)}$. If any kernel address
belongs to the set  $\mathit{addresss(L1)}$, then the program dependency graph
is checked to discover $\mathit{IM1}$ dependent on $\mathit{L1}$.


We note that the original meltdown code involves {\tt flush} instruction
(to flush the probe array from the cache) and {\tt RETSC} instruction (to
time the access of probe array during $\mathit{IM1}$ access). Detecting the
presence of these instructions is straightforward and we remove it from
$\Phi_{meltdown}$ for brevity.






==> commands.tex <==

%\usepackage{xspace}
% Making smaller texttt
% this is necessary to avoid recursion of texttt, put before renew
\let\oldtexttt\texttt 
% xspace is necessary for correct punctuation after the command
\renewcommand{\texttt}[1]{\oldtexttt{\small{#1}}\xspace}
% \footnotesize is also acceptable

\let\oldtextsf\textsf 
% xspace is necessary for correct punctuation after the command
\renewcommand{\textsf}[1]{\oldtextsf{\small{#1}}\xspace}
% \footnotesize is also acceptable


%\usepackage[draft]{fixme} %[final]
% setup for fixme annotations
%\fxsetup{theme=color, inline,nomargin}
%\newcommand{\fix}[1]{\fxnote{#1}\xspace}
% \newcommand{\fixm}[1]{\fxnote[margin, noinline]{#1}\xspace}

%\usepackage{courier}
 %\usepackage{lmodern}
% \usepackage[cmex10]{amsmath}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{color}
\usepackage{graphicx}
%\usepackage{pdfsync} %sync with Skim
\usepackage{listings}          % format code
\usepackage{enumitem}      % adjust spacing in enums
%\usepackage{url}                  % format URLs
% \usepackage[draft]{hyperref}
%\usepackage{cite} 
\usepackage{multirow}
%\usepackage{subcaption}


\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
  \node[shape=circle,draw,inner sep=0.5pt] (char) {#1};}}

\usepackage{balance}
\usepackage{flushend}

\usepackage{microtype} % better alignment for monotype and saves space
\usepackage[htt]{hyphenat}  % to hyphenate monotype words
% gives some font warnings that can safely be ignored

% bug with column alignment when using * floats: 
\usepackage{stfloats}
% \usepackage{fixltx2e} % !!!! do not use this package! Instead of fixing it currupts the alignment 

% IEEETran fixes?
% \ifCLASSOPTIONcompsoc 
%     \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig} 
% \else
    \usepackage[caption=false,font=footnotesize]{subfig} 
% \fi


\usepackage{datetime}


\interdisplaylinepenalty=2500


% Setup for colored code in lstlistings
\definecolor{javared}{rgb}{0.6,0,0} % for strings
\definecolor{javagreen}{rgb}{0.25,0.5,0.35} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc


\lstset{
	%frame=tb,
	language=C,
	%aboveskip=3mm,
	% belowskip=3mm,
	% showstringspaces=false,
	frame=single,
	%columns=flexible,
	basicstyle={\small\ttfamily},
	numbers=left,
	breaklines=true,
	%breakatwhitespace=true,
	tabsize=4,
	columns=flexible
}



%\lstset{
%language=C,
%% basicstyle=\tiny\ttfamily,
%% basicstyle=\scriptsize\sffamily,
%basicstyle=\scriptsize\sffamily,
%xleftmargin=2em,%
%keywordstyle=\color{javapurple}\bfseries,
%stringstyle=\color{javared},
%commentstyle=\color{javagreen},
%morecomment=[s][\color{javadocblue}]{/**}{*/},
%tabsize = 2,
%breaklines=true,
%numbers=left,
%numberstyle=\tiny,
%escapeinside={(*}{*)}, 
%moredelim=[is][\underbar]{`}{`}, % to underline parts of code
%% moredelim=**[is][\color{orange}]{@}{@}, 
%keepspaces=true % for underbar to work correctly
%}
% Setup for colored code in lstlistings end                                       


% %algorithmicx does not have switch statement
\usepackage{algorithm}% http://ctan.org/pkg/algorithm
\PassOptionsToPackage{noend}{algpseudocode}% comment out if want end's to show
\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx 
% \usepackage{algpseudocode}% [noend] % part of algorithmicx package

\newcommand*\Let[2]{\State #1 $\gets$ #2}
\newcommand*\Letn[2]{#1 $\gets$ #2}
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}



% \algsetup{linenosize=\tiny} % does not work
% hack from http://tex.stackexchange.com/questions/145932/reduce-the-line-number-font-size-of-pseudocode
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}


% begin vertical rule patch for algorithmicx (http://tex.stackexchange.com/questions/144840/vertical-loop-block-lines-in-algorithmicx-with-noend-option)
\makeatletter%
\newlength{\continueindent}
\setlength{\continueindent}{4em}

\renewenvironment{algorithmic}[1][0]%
   {%
   \edef\ALG@numberfreq{#1}%
   \def\@currentlabel{\theALG@line}%
   %
   \setcounter{ALG@line}{0}%
   \setcounter{ALG@rem}{0}%
   %
   \let\\\algbreak%
   %
   \expandafter\edef\csname ALG@currentblock@\theALG@nested\endcsname{0}%
   \expandafter\let\csname ALG@currentlifetime@\theALG@nested\endcsname\relax%
   %
   \begin{list}%
      {\ALG@step}%
      {%
      \rightmargin\z@%
      \itemsep\z@ \itemindent\z@ \listparindent2em%
      \partopsep\z@ \parskip\z@ \parsep\z@%
      \labelsep 0.5em \topsep 0.2em%\skip 1.2em 
      \ifthenelse{\equal{#1}{0}}%
         {\labelwidth 0.5em}%
         {\labelwidth 1.2em}%
       \leftmargin\labelwidth \addtolength{\leftmargin}{\labelsep}
      \ALG@tlm\z@%
      }%
      \parshape 2 \leftmargin \linewidth \continueindent \dimexpr\linewidth-\continueindent\relax
   \setcounter{ALG@nested}{0}%
   \ALG@beginalgorithmic%
   }%
   {% end{algorithmic}
   % check if all blocks are closed
   \ALG@closeloops%
   \expandafter\ifnum\csname ALG@currentblock@\theALG@nested\endcsname=0\relax%
   \else%
      \PackageError{algorithmicx}{Some blocks are not closed!!!}{}%
   \fi%
   \ALG@endalgorithmic%
   \end{list}%
   }%
\makeatother


